ACCoRD: A Multi-Document Approach to Generating Diverse Descriptions of Scientific Concepts

Systems that can automatically define unfamiliar terms hold the promise of improving the accessibility of scientific texts, especially for readers who may lack prerequisite background knowledge. However, current systems assume a single "best" description per concept, which fails to account for the many potentially useful ways a concept can be described. We present ACCoRD, an end-to-end system tackling the novel task of generating sets of descriptions of scientific concepts. Our system takes advantage of the myriad ways a concept is mentioned across the scientific literature to produce distinct, diverse descriptions of target scientific concepts in terms of different reference concepts. To support research on the task, we release an expert-annotated resource, the ACCoRD corpus, which includes 1,275 labeled contexts and 1,787 hand-authored concept descriptions. We conduct a user study demonstrating that (1) users prefer descriptions produced by our end-to-end system, and (2) users prefer multiple descriptions to a single "best" description.

==> 2022-03-18-old-dataset-section-before-kyle.tex <==

\section{Task and data set}


\subsection{Task definition} We introduce the task of \taskname. Given a large corpus of scientific documents and a concept to be described (hereafter, \textit{target}), the goal of \taskacronym is to output a set of succinct, self-contained descriptions of the target scientific concept.
While certain automated metrics are possible, such as the number of distinct reference concepts, the complexity and subjectivity of the task imply that manual evaluation based on user preferences is ultimately required.






\subsection{Data set}
\kyle{This section undersells the value of the dataset. We should mention the ``differentia'' property as being captured in the annotation, and this isn't strictly an IE task.  As the dataset is currently described, it sounds like every positive labeled sentence simply needs to have a relational tuple and makes no mention of also requiring rich differentia.}

To support work on \taskacronym, we compile and release Automatic Comparison of Concepts with Relational Descriptions (ACCoRD) corpus.\footnote{Dataset available at \url{https://github.com/allenai/ACCoRD}}
Every description must satisfy the following desiderata: \doug{I like the idea of spelling out desiderata but it might be better to not use a bulleted list but instead just write it in a paragraph.}
\begin{itemize}
    \item length -- 1-2 sentneces max
    \item content -- must contain (1) concept A, (2) concept B, (3) concept A and B are related by a relation $\in \{is-a, compare, part-of, used-for\}$ , (4) must contain a differentia, where... defined as
    \item every positive extractions are allowed to yield multiple concept descriptions \doug{Perhaps give an example of the kind of construction that results in multiple formatted statements.}
\end{itemize}

Our dataset induces diversity among these concept descriptions in two key ways. First, our data set allows for concept descriptions beyond the typical \textit{is-a} relation. The concept descriptions in ACCoRD describe a target scientific concept in terms of another concept using one of four relation types: \emph{is-a}, \emph{compare}, \emph{part-of}, and \emph{used-for}.
Second, a single target concept is allowed to be described in terms of any number of other concepts in the source text.
This means that ACCoRD uniquely allows each positive extraction to yield multiple concept descriptions if a target concept was described in terms of multiple other concepts in the source text, if a single concept pair can be described using multiple relations, or if the extraction contained multiple target concepts.

For example, the extracted text "word embedding is a word representation that captures semantic and syntactic similarities between words. it has been widely utilized for a variety of tasks, such as sentence classification [42] , relation classification [41] , and sentiment analysis [38] , since the introduction of word2vec software." contains the ForeCite concepts \{`word representation', `sentence classification', `relation classification'\}. The extraction, therefore, yields the following hand-authored concept descriptions for 9 unique (target, relation, reference) triples each with a differentia that specifies the relationship between the target and reference concepts: 

\begin{itemize}
    \item (sentence classification, is-a, task), (relation classification, is-a, task) $\rightarrow$ [sentence classification, relation classification] is a task that word embedding has been utilized for since the introduction of word2vec software. 
    \item (sentence classification, compare, relation classification), (sentence classification, compare, sentiment analysis) $\rightarrow$ sentence classification is like [relation classification, sentiment analysis] in that they are tasks that word embedding has been used for since the introduction of word2vec software.
    \item \textit{compare}: (relation classification, compare, sentence classification), (relation classification, compare, sentiment analysis) $\rightarrow$ relation classification is like [sentence classification, sentiment analysis] in that they are tasks that word embedding has been used for since the introduction of word2vec software. 
    \item \textit{used-for}: (word representation, used-for, sentence classification) \dots $\rightarrow$ word representation has been used for [sentence classification, relation classification, sentiment analysis], since the introduction of word2vec software.  
\end{itemize}



\subsection{Data set construction}

\paragraph{Input}
To create our data set, we identified candidate sentences with at least at least one significant CS concept from the abstracts, intros and related works sections of 741 CS papers from S2ORC~\cite{s2orc}, a large corpus of academic papers.
We automatically identify the scientific concepts by performing simple string matching against a high-precision set of concepts extracted from CS papers~\cite{forecite}. We include both 1-sentence and 2-sentence candidates \doug{not clear what these are } \sonia{edited, does this help?} to allow for experiments on the effects of richer context on our task.

\paragraph{Annotation task}
These sentences were labeled as positive if they described a target scientific concept in terms of any other concept. Our dataset includes 2,360 such labeled extractions and were found to have high inter-annotator agreement (Cohen's $\kappa = 0.658$).
For each positive extraction, annotators were additionally asked to use the extracted text to write as many succinct, self-contained descriptions of a target scientific concept in terms of any reference concept in the extraction using one of the four relation types. This means that a single positive extraction could yield multiple concept descriptions if a target concept was described in terms of multiple other concepts in the extracted text, if a single concept pair could be described using multiple relations, or if the extraction contained multiple target concepts. Our dataset contains 1,309 of these hand-authored concept descriptions. 



\subsection{Data set analysis and statistics}

----BASIC STATS-----\\
Number of rows = 3853 \\
Number of extractions with a negative label = 2066 \\
Number of extractions with a positive label = 1275 \\
Number of formatted statements = 1787 \\
--> Number of formatted statements made from an extraction = 1275 \\ 
--> Number of additional formatted statements made from an extraction = 512 \\ 
Number of formatted sentences with no differentia (end with the annotated concept B) = 8 \\
----INTER ANNOTATOR AGREEMENT (BINARY LABELS)-----\\
This dataset was found to have high inter-annotator agreement with a Cohen's $\kappa$ of 0.658. Agreement was computed based on the binary labels.
----OTHER STATS-----\\
tab 1 here: \url{https://docs.google.com/spreadsheets/d/1W1ceJ_5XAxCNbue0UeuVin2Em9B3hR89yv0RCmYgYlk/edit?usp=sharing} \\
(1-sentence setting, 2-sentence setting)
\# of concept b's annotated	567	741 \\
\# of "vague" concept b's (model, system, method, algorithm, dataset)	25	35 \\
\% of concept b's that might be vague	4.41\%	4.72\% \\
\# of concept b's that are forecite	48	117 \\
\% of concept b's that are forecite	8.47\%	15.79\% \\

